Aladdin: Zero-Shot Hallucination of Stylized 3D Assets from Abstract Scene Descriptions

What constitutes the "vibe" of a particular scene? What should one find in "a busy, dirty city street", "an idyllic countryside", or "a crime scene in an abandoned living room"? The translation from abstract scene descriptions to stylized scene elements cannot be done with any generality by extant systems trained on rigid and limited indoor datasets. In this paper, we propose to leverage the knowledge captured by foundation models to accomplish this translation. We present a system that can serve as a tool to generate stylized assets for 3D scenes described by a short phrase, without the need to enumerate the objects to be found within the scene or give instructions on their appearance. Additionally, it is robust to open-world concepts in a way that traditional methods trained on limited data are not, affording more creative freedom to the 3D artist. Our system demonstrates this using a foundation model "team" composed of a large language model, a vision-language model and several image diffusion models, which communicate using an interpretable and user-editable intermediate representation, thus allowing for more versatile and controllable stylized asset generation for 3D artists. We introduce novel metrics for this task, and show through human evaluations that in 91% of the cases, our system outputs are judged more faithful to the semantics of the input scene description than the baseline, thus highlighting the potential of this approach to radically accelerate the 3D content creation process for 3D artists.

==> figures_latex/qualitative_example_kingshand.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.8\textwidth]{figures/kingshand_view1.png}
\caption{ }
\label{fig:kingshand_example}
\end{figure*}



==> figures_latex/system_overview.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.8\textwidth]{figures/system_overview.png}
\caption{ \ian{Create new pipeline figure, with more details into each of the modules. Have it be a one-stop shop for all things method-related.} An overview of the entire system, up to but not including object placement. A skip-connection is missing from \textit{semantic autofill} to \textit{texture painting}, where LLM's can hallucinate large amounts of appearance detail in textual form. \ian{TODO: revamp and focus more on pipeline}}
\label{fig:system_overview}
\end{figure*}


==> shopping_lists/kings_hand.tex <==

\noindent\begin{mdframed}
Input Scene Description : \textbf { characteristic office of the King's Hand in Game of Thrones } 
Semantic shopping list
\begin{enumerate}
\item desk: smooth and polished finish.
\item quill pen: wooden handle and metal tip.new, with a polished finish.
\item inkwell: silver plated with an ornate design and a hinged lid.new, with a glossy finish.
\item book: aged look and embossed with the house sigil.new, with a leathery smell.
\item map: aged look and detailed with antique-style cartography.aged, with a worn look.
\item candles: new, with a fragrant scent.
\item scrolls: aged, with a vintage feel.
\item chair: no visible signs of wear.
\item pillows: slightly worn velvet with minimal fading of the embroidery.
\item blanket: bright and vibrant colors, with no signs of fading.
\item curtains: bright and vibrant colors, with no signs of fading.
\item candles: no signs of melting or discoloring.
\item paintings: no signs of cracking on the canvas, with intricate detailing still intact.
\item bookcases: no visible signs of wear.
\item books: embossed with a crestpristine condition with no signs of wear.
\item scrolls: sealed with the house sigil.slightly creased with a few faded spots.
\item map of westeros: slightly faded in places, but still in good condition.
\item candleholder: inlaid with a dragon motif.no sign of wear, polished to a glossy sheen.
\item rug: no visible signs of wear.
\item candelabras: with ornate gold designs and ruby red jewels.lightly tarnished golden accents, bright ruby red jewels.
\item potted plants: with exotic foliage in a glossy black pot.lush and vibrant foliage.
\item scrolls: with ancient symbols inscribed in gold.well-preserved parchment with neatly written symbols.
\item swords: with ornate hilts and engraved blades.sharp blades, well-polished hilts.
\item throne: no visible signs of wear.
\item pillows: gold and burgundy embroidered with a dragon emblem.rich texture, bright colors.
\item curtains: with golden accents.luxurious feel, brilliantly colored.
\item crown: diamonds and sapphires.shining and flawless.
\item candles: bright and glowing.
\item scepter: shiny and pristine.
\item fireplace: no visible signs of wear.
\item firewood: rusty and charred.
\item fireplace tools: polished and well-used.
\item fireplace mantle: slightly aged and worn.
\item fireplace screen: shiny and well-maintained.
\item fireplace ornament: gleaming and unscathed.
\item banner hanging: no visible signs of wear.
\item ironwork: dark black finish.rustic, vintage finish.
\item tapestry: rich, vibrant colors, with no signs of wear.
\item shields: polished and shining finish.
\item swords: sharp, gleaming blades.
\item candles: unburned, bright wax.
\end{enumerate}
\end{mdframed}

